Keep your memory dump shut: Unveiling data leaks in password managers

Password management has long been a persistently challenging task. This led to the introduction of password management software, which has been around for at least 25 years in various forms, including desktop and browser-based applications. This work assesses the ability of two dozen password managers, 12 desktop applications, and 12 browser-plugins, to effectively protect the confidentiality of secret credentials in six representative scenarios. Our analysis focuses on the period during which a Password Manager (PM) resides in the RAM. Despite the sensitive nature of these applications, our results show that across all scenarios, only three desktop PM applications and two browser plugins do not store plaintext passwords in the system memory. Oddly enough, at the time of writing, only two vendors recognized the exploit as a vulnerability, reserving CVE-2023-23349, while the rest chose to disregard or underrate the issue.

==> Backup_Tables_old/table1.tex <==
\begin{table}[ht]
  \centering
  \begin{tabular}{p{0.13\linewidth} | p{0.85\linewidth}}
    \hline
    \textbf{Scenario} & \textbf{Description} \\
    \hline
    \hline
    S1 & Dump the relevant processes after the user signs up with the product. \\
    \hline
    S2 & Dump the relevant processes following user sign-in and the set of a master password. \\
    \hline
    S3 & Enter the master password and dump the relevant processes. \\
    \hline
    S4 & Manually lock the PM and dump the relevant processes. \\
    \hline
    S5 & The PM is locked automatically; dump the relevant processes. \\
    \hline
    S6 & After creating a new entry password, dump the PM's processes. \\
    \hline
    S7 & While the PM is unlocked, click on a random entry in the corresponding list and dump the relevant processes. \\
    \hline
    S8 & Kill the relevant processes through the task manager, rerun the application without entering the master password and dump the relevant processes. \\
    \hline
  \end{tabular}
  
  \caption{Utilized scenarios per PM application. %The wait time of $\approx$60 sec in S3 and S5 targets the garbage collection process, i.e., how quickly unneeded PM's data are cleared from memory.
  The term ``relevant processes'' in the scenarios refers to either the PM's or the browser's processes in case of a plugin.}
  \label{T:Scenarios}
\end{table}

==> Backup_Tables_old/table2.tex <==
\begin{table}%[H]

\centering
  \begin{tabular}{ | l | c | c | c  c | c  c | c  c | c  c | c  c | c  c |}
    \hline
    %\multirowthead{2}
    {\textbf{Desktop application}} & \multicolumn{1}{c|}{\textbf{S1}} & \multicolumn{1}{c|}{\textbf{S2}} & \multicolumn{2}{c|}{\textbf{S3}} & \multicolumn{2}{c|}{\textbf{S4}} & \multicolumn{2}{c|}{\textbf{S5}} & \multicolumn{2}{c|}{\textbf{S6}} & \multicolumn{2}{c|}{\textbf{S7}} & \multicolumn{2}{c|}{\textbf{S8} } \\ 
    %\cline{2-15} & \multicolumn{14}{c|}{ \centering{{\textbf{M}} \textbf{\textcircled{E}}}} \\ 
    \hline
    \hline
    %& \textbf{M} & \textbf{E} & \textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} \\ \hline
    1Password  & \textcolor{red}{\xmark} & {N/A} & \textcolor{red}{\xmark}  & \cellcolor[gray]{0.8}{\textcolor{red}{\xmark}} & \textcolor{red}{\xmark}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark}  & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    Bitwarden  & {\textcolor{red}{\checkmark}} & {N/A} & {\textcolor{red}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline

    Enpass  & {\textcolor{red}{\checkmark}} & N/A & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\xmark} & \cellcolor[gray]{0.8}\xmark\\ \hline
    
    %LastPass  & -  & - & -  & - & -  & - & -  \\ \hline
    KeePass 2  &{\textcolor{red}{\xmark}}  & {\textcolor{red}{\xmark}}  & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline

    KeePassXC & {\textcolor{red}{\xmark}}  & {N/A}  & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    %\st{DashLane} ? & -   & - & -  & - & -  & - & -  \\ \hline
    Keeper  & {\textcolor{red}{\checkmark}}   & {\xmark} & {\textcolor{red}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {} & \cellcolor[gray]{0.8}   & {} & \cellcolor[gray]{0.8}  & {\xmark} & \cellcolor[gray]{0.8}\xmark  & {} & \cellcolor[gray]{0.8} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    Kaspersky  & {\textcolor{red}{\checkmark}}  & {\textcolor{red}{\xmark}}  & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline

    Nordpass & {\textcolor{red}{\xmark}} &  {\textcolor{red}{\checkmark}} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\textcolor{red}{\xmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\xmark} & {\xmark}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} & {\textcolor{red}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark}  & {\xmark} & \cellcolor[gray]{0.8}\xmark\\ \hline

    Passwarden & {\textcolor{blue}{\xmark}} &  {\textcolor{blue}{\checkmark}} & {\textcolor{blue}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & {\textcolor{blue}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & {\textcolor{blue}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & {\textcolor{blue}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & {\textcolor{blue}{\checkmark}}  & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark}  & {\xmark} & \cellcolor[gray]{0.8}\xmark\\ \hline

    PasswordBoss & {\xmark} & {\xmark} &  {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {}  & \cellcolor[gray]{0.8}  & {\xmark} & \cellcolor[gray]{0.8}\xmark\\ \hline

    RoboForm  & {\xmark}  &  {\xmark}  &  {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {}  & \cellcolor[gray]{0.8} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    StickyPassword &{\xmark}  &  {\xmark}   & {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {}  & \cellcolor[gray]{0.8} & {\xmark}  & \cellcolor[gray]{0.8}\xmark & {}  & \cellcolor[gray]{0.8} & {\xmark} & \cellcolor[gray]{0.8}\xmark \\ \hline

  
  \end{tabular}

  \caption{Results for standalone PMs. The results for master and \colorbox{lightgray}{entry} password are given in white and lightgrey background, respectively (\checkmark: password leak, \xmark: no password leak). \textcolor{red}{tz:I want to repeat S1 and S2 for the first 5 desktop apps. This is why you see sporadically red checkmarks. I have also done this for S6. Vyron if you have time please do the same for the rest (i.e., Keeper, Passwarden and bellow).} \gk{Yes}. \textcolor{blue}{vk: I think there is no need for N/A in S1 and S2, instead i removed the entry password column (grey).}}
  
  \label{results-apps}%
\end{table}

==> Backup_Tables_old/table3.tex <==
\begin{table}[ht]
  
\centering
  \begin{tabular}{ | l | c | c | c c | c c | c c | c c | c c | c c |}
    \hline
    %\multirowthead{2}
    {\textbf{Desktop application}} & \multicolumn{1}{c|}{\textbf{S1}} & \multicolumn{1}{c|}{\textbf{S2}} & \multicolumn{2}{c|}{\textbf{S3}} & \multicolumn{2}{c|}{\textbf{S4}} & \multicolumn{2}{c|}{\textbf{S5}} & \multicolumn{2}{c|}{\textbf{S6}} & \multicolumn{2}{c|}{\textbf{S7}} & \multicolumn{2}{c|}{\textbf{S8}}\\ 
    %\cline{2-15} & \multicolumn{14}{c|}{ \centering{{\textbf{M}} \textbf{\textcircled{E}}}} \\ 
    \hline 
    \hline 
    1Password  & - & 2? & - & \cellcolor[gray]{0.8}- &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}21 & - & \cellcolor[gray]{0.8}- & \multicolumn{2}{c|}{ - }\\ \hline

    BitWarden  & \textcolor{red}{15}  &  - & 1 & \cellcolor[gray]{0.8}1 &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}11 & 4 &  \cellcolor[gray]{0.8}2 & \multicolumn{2}{c|}{ - }\\ \hline

    Enpass  & \textcolor{red}{1}  & - & - & \cellcolor[gray]{0.8}- &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}1 & - & \cellcolor[gray]{0.8}1 & \multicolumn{2}{c|}{ - }\\ \hline

    KeePass 2  & - &  2? & - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & - & \multicolumn{2}{c|}{ - }\\ \hline

    KeePassXC  & - & - &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- &  - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}- &  - & - & \multicolumn{2}{c|}{ - } \\ \hline

    Keeper & \textcolor{red}{25}  & - & \textcolor{red}{10} & \cellcolor[gray]{0.8}\textcolor{red}{13}  & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & { \cellcolor[gray]{0.8}- }  & - & - & \multicolumn{2}{c|}{ - }\\ \hline

    Kaspersky & \textcolor{red}{1} & 2? & - & \cellcolor[gray]{0.8}- &  - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}- &  2 & \cellcolor[gray]{0.8}- & - & - &  \multicolumn{2}{c|}{ - } \\ \hline

    Nordpass & - &  2 & \textcolor{red}{1} & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & 1 & \cellcolor[gray]{0.8}21 &  \textcolor{red}{1} & \cellcolor[gray]{0.8}\textcolor{red}{4} & \multicolumn{2}{c|}{ - } \\ \hline

    Passwarden & - &  \textcolor{blue}{1} & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} &  \cellcolor[gray]{0.8}\textcolor{blue}{15} &  \textcolor{blue}{2} &  \cellcolor[gray]{0.8}\textcolor{blue}{8} & \multicolumn{2}{c|}{ - } \\ \hline

    PasswordBoss & - & - & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- &  - &  - & \multicolumn{2}{c|}{ - }  \\ \hline

    RoboForm  & -  & - & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & - & \multicolumn{2}{c|}{ - } \\ \hline  

    StickyPassword & -  & - & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}- & - & - & \multicolumn{2}{c|}{ - }\\ \hline
     
  \end{tabular}
  \caption{Number of password instances found in the dump files of each standalone PM product. The results for master and \colorbox{lightgray}{entry} password are given in white and lightgrey background, respectively. \textcolor{blue}{In s6 the newly created entry password appears more than the already existing entry passwords (Passwarden 15 refers to the sum, 12 times the new entry, and 3 time the old).}}
  \label{T:PM:Desktop:Results}
\end{table}

==> Backup_Tables_old/table4.tex <==
\begin{table}[htbp]
  \centering
  \begin{tabular}{ | l | c c | c c | c c | c c | c c | c c | c c | c c |}
    \hline
    
    {\textbf{Browser plugin}} & \multicolumn{2}{c|}{\textbf{S1}} & \multicolumn{2}{c|}{\textbf{S2}} & \multicolumn{2}{c|}{\textbf{S3}} & \multicolumn{2}{c|}{\textbf{S4}}& \multicolumn{2}{c|}{\textbf{S5}}& \multicolumn{2}{c|}{\textbf{S6}}& \multicolumn{2}{c|}{\textbf{S7}} & \multicolumn{2}{c|}{\textbf{S8}}\\ 
    \hline 
    \hline 
    1Password  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   & \cellcolor[gray]{0.8}  & \xmark  & \cellcolor[gray]{0.8}\xmark  &   & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark\\ \hline

    Avira  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   \multicolumn{2}{c|}{ N/A }  & \xmark  & \cellcolor[gray]{0.8}\xmark  & \multicolumn{2}{c|}{ N/A } & \xmark & \cellcolor[gray]{0.8}\xmark \\   \hline

    Bitdefender  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   & \cellcolor[gray]{0.8}  & \xmark  & \cellcolor[gray]{0.8}\xmark  &   & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark \\ \hline

    Bitwarden  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   & \cellcolor[gray]{0.8}  & \xmark  & \cellcolor[gray]{0.8}\xmark  &   & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    Dashlane  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   & \cellcolor[gray]{0.8}  & \xmark  & \cellcolor[gray]{0.8}\xmark  &   & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark \\ \hline
        
    Ironvest  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   \multicolumn{2}{c|}{ N/A }  & \xmark  & \cellcolor[gray]{0.8}\xmark  & \multicolumn{2}{c|}{ N/A } & \xmark & \cellcolor[gray]{0.8}\xmark \\\hline
    
    LastPass  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   \multicolumn{2}{c|}{ N/A }  & \xmark  & \cellcolor[gray]{0.8}\xmark  &  \multicolumn{2}{c|}{ N/A } & \xmark & \cellcolor[gray]{0.8}\xmark \\ \hline
    
    Norton  & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   \multicolumn{2}{c|}{ N/A }  & \xmark  & \cellcolor[gray]{0.8}\xmark  & \multicolumn{2}{c|}{ N/A } & \xmark & \cellcolor[gray]{0.8}\xmark \\  \hline
    
    RoboForm   & \xmark & \cellcolor[gray]{0.8}\xmark  & \xmark & \cellcolor[gray]{0.8}\xmark  &  & \cellcolor[gray]{0.8}  &  & \cellcolor[gray]{0.8}  &   \multicolumn{2}{c|}{ N/A }  & \xmark  & \cellcolor[gray]{0.8}\xmark  &  \multicolumn{2}{c|}{ N/A } & \xmark & \cellcolor[gray]{0.8}\xmark   \\ \hline

  \end{tabular}
  \caption{Results for PM browser plugins. The results for master and \colorbox{lightgray}{entry} password are given in white and lightgrey background, respectively (\checkmark: password leak, \xmark: no password leak, N/A: not applicable; the plugin does not provide a lock feature (S5) or the plugin does not require entering the master password after reopening the browser (S7).}
  \label{T:PM:Plugins:Results}
\end{table}

==> Tables/table2.tex <==
\begin{table}[ht]

\centering
  \begin{tabular}{ | l | c  c | c  c | c  c | c  c | c  c | c  c |}
    \hline
    %\multirowthead{2}
    {\textbf{PM App}} & \multicolumn{2}{c|}{\textbf{S1}} & \multicolumn{2}{c|}{\textbf{S2}} & \multicolumn{2}{c|}{\textbf{S3}} & \multicolumn{2}{c|}{\textbf{S4}} & \multicolumn{2}{c|}{\textbf{S5}} & \multicolumn{2}{c|}{\textbf{S6} } \\ 
    %\cline{2-15} & \multicolumn{14}{c|}{ \centering{{\textbf{M}} \textbf{\textcircled{E}}}} \\ 
    \hline
    \hline
    %& \textbf{M} & \textbf{E} & \textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} &\textbf{M} & \textbf{E} \\ \hline
    1Password & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline
    
    Bitwarden & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ \hline

    Enpass  & \xmark & \cellcolor[gray]{0.8}\xmark & \xmark & \cellcolor[gray]{0.8}\xmark & \xmark & \cellcolor[gray]{0.8}\xmark & \xmark & \cellcolor[gray]{0.8}\checkmark & \xmark & \cellcolor[gray]{0.8}\checkmark & \xmark & \cellcolor[gray]{0.8}\xmark\\ 
    \hline

    Kaspersky & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline
    
    %LastPass  & -  & - & -  & - & -  & - & -  \\ \hline
    KeePass 2 & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline

    KeePassXC & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline
    
    %\st{DashLane} ? & -   & - & -  & - & -  & - & -  \\ \hline
    Keeper & \textcolor{red}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{red}{\checkmark} &  & \cellcolor[gray]{0.8} &  & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark &  & \cellcolor[gray]{0.8} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline

    Nordpass & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark}  & \xmark & \cellcolor[gray]{0.8}\xmark\\ 
    \hline

    Passwarden & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark}  & \xmark & \cellcolor[gray]{0.8}\xmark\\ 
    \hline

    PasswordBoss & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline

    RoboForm & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \textcolor{blue}{\checkmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\checkmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline
    
    StickyPassword & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \textcolor{blue}{\xmark} & \cellcolor[gray]{0.8}\textcolor{blue}{\xmark} & \xmark & \cellcolor[gray]{0.8}\xmark \\ 
    \hline

  \end{tabular}

  \caption{Results for standalone PMs. Master and \colorbox{lightgray}{entry} cleartext password leaks are given in white and lightgrey background, respectively (\checkmark: password leak, \xmark: no password leak).}
  
  \label{results-apps}%
\end{table}

==> Tables/table3.tex <==
\begin{table}[ht]
  
\centering
  \begin{tabular}{ | l | c | c | c c | c c | c c | c c | c c | c c |}
    \hline
    %\multirowthead{2}
    {\textbf{PM App}} & \multicolumn{2}{c|}{\textbf{S1}} & \multicolumn{2}{c|}{\textbf{S2}} & \multicolumn{2}{c|}{\textbf{S3}} & \multicolumn{2}{c|}{\textbf{S4}} & \multicolumn{2}{c|}{\textbf{S5}} & \multicolumn{2}{c|}{\textbf{S6}}\\ 
    %\cline{2-15} & \multicolumn{14}{c|}{ \centering{{\textbf{M}} \textbf{\textcircled{E}}}} \\ 
    \hline 
    \hline 
    1Password & \textcolor{blue}{10} & \cellcolor[gray]{0.8}- & \textcolor{blue}{2} & \cellcolor[gray]{0.8}- & \textcolor{blue}{2} & \cellcolor[gray]{0.8}- & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{4} & \textcolor{blue}{1} & \cellcolor[gray]{0.8}- & \multicolumn{2}{c|}{ - }\\ 
    \hline

    BitWarden & \textcolor{blue}{8} & \cellcolor[gray]{0.8}\textcolor{blue}{2} &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & \textcolor{blue}{1} & \cellcolor[gray]{0.8}\textcolor{blue}{7} & \textcolor{blue}{1} &  \cellcolor[gray]{0.8}\textcolor{blue}{3} & \multicolumn{2}{c|}{ - }\\ \hline

    Enpass & - & \cellcolor[gray]{0.8}- &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}1 & - & \cellcolor[gray]{0.8}1 & \multicolumn{2}{c|}{ - }\\ \hline

    Kaspersky & - & \cellcolor[gray]{0.8}- &  - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- &  \multicolumn{2}{c|}{ - } \\ \hline

    KeePass 2 & - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & \multicolumn{2}{c|}{ - }\\ \hline

    KeePassXC &  - &  \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- &  - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}\textcolor{blue}{1} &  - & \cellcolor[gray]{0.8}- & \multicolumn{2}{c|}{ - } \\ \hline

    Keeper & \textcolor{red}{10} & \cellcolor[gray]{0.8}\textcolor{red}{13}  & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & { \cellcolor[gray]{0.8}- }  & - & - & \multicolumn{2}{c|}{ - }\\ \hline

    Nordpass & \textcolor{blue}{2} & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}\textcolor{blue}{24} & \textcolor{blue}{4} & \cellcolor[gray]{0.8}\textcolor{blue}{19} & \multicolumn{2}{c|}{ - } \\ \hline

    Passwarden & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} & \cellcolor[gray]{0.8}\textcolor{blue}{3} & \textcolor{blue}{2} &  \cellcolor[gray]{0.8}\textcolor{blue}{12} &  \textcolor{blue}{2} &  \cellcolor[gray]{0.8}\textcolor{blue}{8} & \multicolumn{2}{c|}{ - } \\ \hline

    PasswordBoss & - & \cellcolor[gray]{0.8}\textcolor{blue}{8} & - & \cellcolor[gray]{0.8}\textcolor{blue}{4} & - & \cellcolor[gray]{0.8}\textcolor{blue}{1} & - & \cellcolor[gray]{0.8}\textcolor{blue}{11} &  - &  \cellcolor[gray]{0.8}\textcolor{blue}{7} & \multicolumn{2}{c|}{ - } \\ \hline

    RoboForm & \textcolor{blue}{1} & \cellcolor[gray]{0.8}\textcolor{blue}{1} & \textcolor{blue}{1} & \cellcolor[gray]{0.8}- & \textcolor{blue}{2} & \cellcolor[gray]{0.8}- & \textcolor{blue}{1} & \cellcolor[gray]{0.8}\textcolor{blue}{2} & \textcolor{blue}{1} & \cellcolor[gray]{0.8}\textcolor{blue}{2} & \multicolumn{2}{c|}{ - } \\ \hline  

    StickyPassword & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}-  & - & \cellcolor[gray]{0.8}- & - & \cellcolor[gray]{0.8}- & \multicolumn{2}{c|}{ - }\\ \hline
     
  \end{tabular}
  \caption{Number of password instances found in the dump files of each standalone PM product. The results for master and \colorbox{lightgray}{entry} password are given in white and lightgray background, respectively.}
  \label{T:PM:Desktop:Results}
\end{table}

%1password: Notes: Only at the time of creating an entry password it leaks it. passwords were found in different .dmp files.
%Roboform: When it locks either automatically or manually it deletes entry passwords, while when open the same passwords are visible
%PasswordBoss: only leaks entry pass
%Passwarden: leaks everything in every scenario except 6
%KeePassXC: only when you create a new entry pass it leaks (s4).
%bitwarden: only leaks when unlocked both master and entries, and in the same file.
%enpass: only when there is some interaction with some entry password (s4, s5) it leaks it.
%nordpass: only when the app is unlocked it leaks, in different files and the entry pass can be found only when there is interaction with it (s4, s5). The interesting here is that the master pass can be found in s1 and s5 but not in s4 when the new entry is created (doubled checked with multiple exps).
